Multimodal Dialogue Management for Multiparty Interaction with Infants

We present dialogue management routines for a system to engage in multiparty agent-infant interaction. The ultimate purpose of this research is to help infants learn a visual sign language by engaging them in naturalistic and socially contingent conversations during an early-life critical period for language development (ages 6 to 12 months) as initiated by an artificial agent. As a first step, we focus on creating and maintaining agent-infant engagement that elicits appropriate and socially contingent responses from the baby. Our system includes two agents, a physical robot and an animated virtual human. The system's multimodal perception includes an eye-tracker (measures attention) and a thermal infrared imaging camera (measures patterns of emotional arousal). A dialogue policy is presented that selects individual actions and planned multiparty sequences based on perceptual inputs about the baby's internal changing states of emotional engagement. The present version of the system was evaluated in interaction with 8 babies. All babies demonstrated spontaneous and sustained engagement with the agents for several minutes, with patterns of conversationally relevant and socially contingent behaviors. We further performed a detailed case-study analysis with annotation of all agent and baby behaviors. Results show that the baby's behaviors were generally relevant to agent conversations and contained direct evidence for socially contingent responses by the baby to specific linguistic samples produced by the avatar. This work demonstrates the potential for language learning from agents in very young babies and has especially broad implications regarding the use of artificial agents with babies who have minimal language exposure in early life.

==> Sections/Components.tex <==
%components 
%( eyetracker - thermal imaging - robot - avatar - behavioral woz input )
%Figure \ref{fig:components} shows a sketch of the physical arrangement of the components in the experimental setup. ({\color{red}TODO: redraw })
Going through details of the components is beyond the scope of this paper. But a brief yet sufficient explanation will be given about each of them such that the overall design can be understood.

\begin{comment}
	\begin{figure}[h]
	\centering
	\includegraphics[width=3in]{Figures/components}
	\caption{Physical arrangements of system components}
	\label{fig:components}
	\end{figure}
\end{comment}


\subsubsection{Eye-tracker}
Infant's gaze direction as a behavioral response was used as an input to the system. A Tobii Pro X3-120 EPU was used to capture the baby's eye-gaze at the rate of 60 HZ using a customized python script. 4 different area of interests (AOI) were defined: Robot, Avatar, In-between and Outside. We took into account the AOIs as well as the fixation on the target as an indicator of baby's focus of interest. Figure \ref{fig:AOI} shows the relative setup of the AOIs with respect to the visible display area. We performed a majority vote paradigm every half second (60 data points) to determine the area of interest. A calibration process was done in the beginning of the experiment to accommodate the program to the physical setup and the relative coordination of the baby's eyes, targets and the tracker. 

\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{Figures/AOI}
\caption{AOI coordinations in relation with active display area from the infant's point of view}
\label{fig:AOI}
\end{figure}


\subsubsection{Thermal Infrared Imaging}
\begin{comment}
Thermal IR imaging allows the system to detect subtle changes in the infant’s internal state, which are significant for discriminating when the infant is engaged with the interaction. Facial thermal patterns depend on subcutaneous vessels transporting blood heat, and these vessels regulate blood flow via local vascular resistance (vasodilation and vasoconstriction) and arterial pressure [5, 46]. Therefore, by recording the dynamics of the facial cutaneous temperature, it is possible to assess autonomic nervous system activity and infer the subject’s emotional state [47, 22, 43, 46]. We choose the nasal tip as the salient region of interest (ROI) for assessing the psychophysiological activity of the infants,because of its strict neurovascular relationship with adrenergic activity associated with expression of emotional states [22, 43]. The nose tip’s average temperature was extracted from each frame thus obtaining a temperature signal in real time. The dynamics of the temperature was used to classify the arousal state of the infants by assuming that a decrease of temperature is linked with a sympathetic-like response (associated with distress and disengagement) whereas its increase is due to a parasympathetic prevalence on the subject autonomic state (related with interest and social engagement)[43]. Thermal IR imaging is performed by means of a digital IR thermal camera FLIR A655sc (640 x 480 microbolometer FPA, NETD: < 30 mK @ 30 °C, sampling rate: 50 Hz). In order to preserve the ecology of the recording in challenging situations like experiments with infants and toddlers, the facial ROIs need to be automatically recognized and tracked in all the frames of the thermal video. The original solution developed includes three different processes: i) automatic recognition of facial landmarks in the visible domain using the Open Face library [4]; ii) frame-to-frame tracking of the ROIs in the visible domain by referencing them with respect to the facial landmarks; iii) co-registration of the visible ROIs with their corresponding ROIs in the thermal videos.
\end{comment}

We used facial thermal patterns for capturing the infant's internal state. 

\subsubsection{Robot}
The robot is based on the op;en-source Maki platform from Hello Robot. We performed some modification like enlarging the eyes and adding hair to it to make it more baby-friendly according to our specific experimental needs. The main purpose of the Robot is to shift the baby's directional attention to the Avatar since it has been shown that infants are capable of following gaze direction. The robot has an articulated head (pan left/right, tilt up/down), articulated eyes (pan left/right, tilt up/down) and eyelids (open/close). Figure \ref{fig:maki} shows the robot used in the study. { \color{red} (Remove th background )} 

\begin{figure}[h]
	\centering
	\includegraphics[width=3in]{Figures/maki}
	\caption{Maki Robot}
	\label{fig:maki}
\end{figure}

\subsubsection{Avatar}

\subsubsection{Kinect}
In order to maintain a responsive system, it was crucial to have a visual perception component to capture the communicative and social behaviors of the infant such as hand clapping, pointing, reaching and etc.  The challenge we face is that most of the current tracking system such as Kinect use models which are trained on adults anatomy thus they do not work as properly on infants due to their fundamental differences in posture and morphology. Furthermore, in our experiment, the baby is sitting on parent's lap  so this will bring additional complications for tracking system which are mostly trained on full body postures. To address these issues, we tend to collect data from these experiments with the hope of having enough data for future customizing models to correspond to our specific demands with respect to the experiment setup. 
\subsubsection{Behavioral GUI}




==> Sections/results.tex <==
%results 

